Geometric theory of the natural optical activity in noncentrosymmetric metals

This is a PhD dissertation. Ignited by the chiral anomaly of recently discovered Weyl (semi-)metals, we study the chiral magnetic effect and the natural optical activity of noncentrosymmetric metals. Both phenomena are related to the linear-in-$\mathbf{q}$ spatial dispersion of the optical conductivity tensor, and can be calculated within the formalism of the semiclassical kinetic equation. Therefore, we calculate the dispersion of optical conductivity up to the linear order of the wave vector, in the low frequency regime, with both the semiclassical Boltzmann equation and the Kubo formula. The two different methods of calculation provide us the same result. In this result, the static and dynamic chiral magnetic effects are revealed to have different origin: one comes from topology, related to Berry monopoles, and the other has a geometric origin, which is determined by the orbital magnetic moment. The Faraday rotation of the polarization of light transmitted through a slab of the sample provides us the most direct way to measure the magnitude of dynamic chiral magnetic effect. We develop an effective medium theory for electromagnetic wave propagating through gapless nonuniform systems, to calculate macroscopic sample inhomogeneities induced corrections to the chiral magnetic conductivity. We show that, in metals with low carrier density, the way in which macroscopic fluctuations of the local conductivity affect the frequency dependent of the measured optical polarization rotation angle: by creating a sharp feature near the plasma edge, which can be detected by experiments. Then we narrow down our research a bit further to the current induced magnetization.

==> Makefile <==
### ====================================================================
### Makefile for University of Utah Sample Thesis
###
### Current target list:
###	all			make .dvi file
###	aux			make .aux file
###	bbl			make .bbl file
###	check			doubled-word, spelling, and syntax checks
###	clean			remove intermediate automatically-created
###				files
###	clobber			same as distclean
###	distclean		remove most automatically-created files
###	dvi			make .dvi file
###	dw			make double-word check
###	FRC			dummy target
###	install			install files on system (dummy target)
###	maintainer-clean	remove absolutely everything that make can
###				build
###	mostlyclean		same as clean
###	pdf			make PDF file(s)
###	ps			make PostScript file(s)
###	spell			make spelling check
###	sample-thesis-0		same as sample-thesis-0.dvi
###	sample-thesis-0.aux
###	sample-thesis-0.dvi
###	sample-thesis-0.bbl
###	sample-thesis-0.pdf
###	sample-thesis-0.ps
###	sample-thesis-0.toc
###	uninstall		uninstall installed files (dummy target)
###
### [16-Mar-2016] -- update for TeX Live and default of PDF output
### [28-May-2001] -- update for LaTeX2e
### [06-Jul-1993]
### ====================================================================

BIBTEX          = bibtex

CAT		= /bin/cat

CP		= /bin/cp -p

DETEX           = detex -n

### Use whichever of these you have:
DISTILL		= distill
DISTILL		= ps2pdf

### The dvips-type1 script is a local wrapper that ensures that Type 1
### outline fonts are used, instead of bitmap fonts, because Acrobat
### Reader does a poor job of displaying the latter.
DVIPS		= dvips-type1
DVIPS		= dvips

### dw is available at ftp://ftp.math.utah.edu/pub/misc/dw.tar.gz
DW		= dw

### Filter to tweak .idx file entries.  Usually, this would be
### a sed script, but for now, it is just a dummy that copies
### its input to its output without changes
FIXIDX		= $(SED) -e 's/\[-\]/-/g' -e 's/\\ / /g'
FIXIDX		= $(CAT)

FGREP		= fgrep

LACHECK		= lacheck

### Many sites call this latex, with the old 2.09 version available as
### latex209, or not at all.  At the University of Utah Mathematics
### department, latex is always 2.09, and latex2e is 2e.
LATEX           = latex2e

### TeX Live name
LATEX           = latex

MAKEINDEX	= makeindex

MAKEINDEXFLAGS	= -c

MV		= /bin/mv

### TeX Live name
PDFLATEX	= pdflatex

RM              = rm -f

SED             = sed

SHELL		= /bin/sh

### We used to use "spell +file.sok" on Sun Solaris, but GNU/Linux
### systems use a different syntax for that command.  Instead, we use
### another spelling program, with the -l option to list spelling
### exceptions, and later below, with the "-p $(THESIS).sok" option to
### supply a private dictionary for this student thesis.
SPELL		= hunspell -l

TOUCH		= touch

TRUE		= true

### ====================================================================
### Personal files to be updated for each student.  It is CRITICAL that
### these lists be complete, because they are dependencies on which
### correct typesetting depends.  If a dependent file is missing here,
### then a change to that file would not cause typesetting to be done
### on the next "make" command!

EPSFILES	= fig1.eps			\
		  fig2.eps 			\
		  fig3.eps

FIGFILES	= fig1.tex			\
		  fig2.tex 			\
		  fig3.tex

PDFFILES	= fig1.pdf			\
		  fig2.pdf 			\
		  fig3.pdf

STYFILES	= amssymb.sty			\
		  amssymbols.sty		\
		  diagram.sty			\
		  dissertationapproval.sty	\
		  lamsarrow.sty			\
		  mythesis.sty			\
		  rgb.sty			\
		  tgrind.sty			\
		  uuthesis-2016-h.sty		\
		  uuthesis-color-headings.sty

TEXFILES        = abstract.tex			\
		  acknowledge.tex		\
		  chap1.tex			\
		  chap2.tex			\
		  chap3.tex			\
		  chap4.tex			\
		  appa.tex			\
		  appb.tex			\
		  appc.tex			\
		  notation.tex

THESIS		= sample-thesis-0

TOPFILE		= $(THESIS).tex

.SUFFIXES:

### ====================================================================

### all:	dvi
all:	pdf

aux:	$(THESIS).aux

bbl:
	-$(BIBTEX) $(THESIS)

bbl-ind-toc:
	-$(MAKE) bbl
	-$(MAKE) indexes
	-$(MAKE) toc

check:	 dw spell syntax-check

clean:
	-$(RM) *.blg
	-$(RM) *.dvi*
	-$(RM) *.dw
	-$(RM) *.ilg
	-$(RM) *.log
	-$(RM) *.o
	-$(RM) *.ser
	-$(RM) *.tmp
	-$(RM) *.old
	-$(RM) *~
	-$(RM) \#*
	-$(RM) core

clobber:	distclean

distclean:	mostlyclean
	-$(RM) *.aux
	-$(RM) *.bbl
	-$(RM) *.idx
	-$(RM) *.ind
	-$(RM) *.toc
	-$(RM) *.lof
	-$(RM) *.lot

dvi:	$(THESIS).dvi

### NB: Because we do "\input{}" on the extra indexes, they MUST exist:
### create empty files if they do not.
dvi-pass:
	test -f $(THESIS)-bioname.ind || $(TOUCH) $(THESIS)-bioname.ind
	test -f $(THESIS)-fsfname.ind || $(TOUCH) $(THESIS)-fsfname.ind
	-$(LATEX) $(THESIS).tex
	-$(MAKE) bbl-ind-toc

dw:
	-$(RM) $(THESIS).dw
	@echo '==================== doubled words ===================='
	for f in $(TEXFILES) $(TOPFILE) ; 		\
	do						\
		echo ===== $$f ===== ;			\
		echo ===== $$f ===== >> $(THESIS).dw ;	\
		$(DETEX) $$f  | $(DW) >> $(THESIS).dw ; \
	done

### dummy target for force make to make a rule
FRC:

#indexes:	$(THESIS).ind $(THESIS)-bioname.ind $(THESIS)-fsfname.ind
indexes:

install:
	@echo There is nothing to install for this package

maintainer-clean:	distclean
	@echo "This command is intended for maintainers to use;"
	@echo "it deletes files that may require special tools to rebuild."
	-$(RM) $(THESIS).pdf $(THESIS).ps

mostlyclean:	clean

### NB: Because we do "\input{}" on the extra indexes, they MUST exist:
### create empty files if they do not.
pdf-pass:
	test -f $(THESIS)-bioname.ind || $(TOUCH) $(THESIS)-bioname.ind
	test -f $(THESIS)-fsfname.ind || $(TOUCH) $(THESIS)-fsfname.ind
	-$(PDFLATEX) $(THESIS).tex
	-$(MAKE) bbl-ind-toc

pdf:	$(THESIS).pdf

ps:	$(THESIS).ps

spell:	$(TEXFILES) $(TOPFILE)
	-if [ ! -f $(THESIS).sok ] ; then touch $(THESIS).sok ; fi
	@echo '==================== spelling exceptions ===================='
	for f in $(TEXFILES) $(TOPFILE) ;						\
	do								\
		echo ===== $$f ===== ;					\
		g=`basename $$f .tex` ;					\
		$(DETEX) $$f  | $(SPELL) -p $(THESIS).sok > $$g.ser;	\
		if [ -s $$g.ser ] ;					\
		then cat $$g.ser ;					\
		else $(RM) $$g.ser ;					\
		fi ;							\
	done

syntax-check:
	$(LACHECK) $(THESIS).tex

thesis:	$(THESIS).pdf

toc:	$(THESIS).toc

$(THESIS).aux:
	-if [ ! -f $(THESIS).aux ] ; then touch $(THESIS).aux ; fi

### NB: Because of extensive cross-referencing in the thesis, and in
### the bibliography entries, we need FOUR complete passes to reach
### consistency!
$(THESIS).dvi:	Makefile $(THESIS).bbl $(EPSFILES) $(FIGFILES) $(STYFILES) $(TEXFILES) $(TOPFILE)
	-$(MAKE) dvi-pass
	-$(MAKE) dvi-pass
	-$(MAKE) dvi-pass
	-$(MAKE) dvi-pass

### Rigorously, the .bbl file also depends on the .aux file, but
### because that gets created anew each LaTeX run, a dependency on the
### .aux file causes $(THESIS).dvi or $(THESIS).pdf to be remade
### unnecessarily, so we suppress that dependency.
### $(THESIS).bbl:	$(THESIS).bib $(THESIS).aux

$(THESIS).bbl:	$(THESIS).bib
	-$(MAKE) $(THESIS).aux
	-$(BIBTEX) $(THESIS)

### NB: We remove the fsfname entries from the topic index, but leave
### the bioname ones!
$(THESIS).ind:	FRC $(THESIS).idx $(THESIS).ist
	$(MV) $(THESIS).idx $(THESIS).idx.old
	$(FIXIDX) < $(THESIS).idx.old > $(THESIS).idx
	-$(FGREP) -v fsfname $(THESIS).idx | $(MAKEINDEX) $(MAKEINDEXFLAGS) -s $(THESIS).ist > $@

### NB: Because of extensive cross-referencing in the thesis, and in
### the bibliography entries, we need FOUR complete passes to reach
### consistency!
$(THESIS).pdf:	Makefile $(THESIS).bbl $(FIGFILES) $(PDFFILES) $(STYFILES) $(TEXFILES) $(TOPFILE)
	-$(MAKE) pdf-pass
	-$(MAKE) pdf-pass
	-$(MAKE) pdf-pass
	-$(MAKE) pdf-pass

$(THESIS).ps:	$(THESIS).dvi
	$(DVIPS) -o $@ $?

### This will strip the sections from appearing in the table of contents.
# $(THESIS).toc:	FRC
$(THESIS).toc:
#	$(CP) $(THESIS).toc $(THESIS).toc.old
#	$(SED) '/[AB]\.[12]/d' <$(THESIS).toc.old >$(THESIS).toc

$(THESIS)-fsfname.ind:	FRC
	-$(FGREP) fsfname $(THESIS).idx | $(FGREP) -v '|see' | $(MAKEINDEX) -c -s $(THESIS).ist > $@

$(THESIS)-bioname.ind:	FRC
	-$(FGREP) bioname $(THESIS).idx | $(FGREP) -v '|see' | $(MAKEINDEX) -c -s $(THESIS).ist > $@

uninstall:
	@echo There is nothing to uninstall for this package

2:
	-$(MAKE) pdf-pass
	-$(MAKE) pdf-pass


==> abstract.tex <==
%%% -*-LaTeX-*-
%%% This is the abstract for the thesis. 
%%% It is included in the top-level LaTeX file with
%%%
%%%    \preface    {abstract} {Abstract}
%%%
%%% The first argument is the basename of this file, and the
%%% second is the title for this page, which is thus not 
%%% included here.  
%%%
%%% The text of this file should be about 350 words or less.
Ignited by the chiral anomaly of recently discovered Weyl (semi-)metals, we study the chiral magnetic effect and the natural optical activity of noncentrosymmetric metals.  Both phenomena are related to the linear-in-$\mathbf{q}$ spatial dispersion of the optical conductivity tensor, and can be calculated within the formalism of the semiclassical kinetic equation. Therefore, we calculate the dispersion of optical conductivity up to the linear order of the wave vector, in the low frequency regime, with both the semiclassical Boltzmann equation and the Kubo formula. The two different methods of calculation provide us the same result. In this result, the static and dynamic chiral magnetic effects are revealed to have different origin: one comes from topology, related to Berry monopoles, and the other has a geometric origin, which is determined by the orbital magnetic moment.  The Faraday rotation of the polarization of light transmitted through a slab of the sample provides us the most direct way to measure the magnitude of dynamic chiral magnetic effect. %In order to verify whether the symmetric local optical conductivity affect the Faraday rotation angle or not,
 We develop an effective medium theory for electromagnetic wave propagating through gapless nonuniform systems, to calculate macroscopic sample inhomogeneities induced corrections to the chiral magnetic conductivity. We show that, in metals with low carrier density, the way in which macroscopic fluctuations of the local conductivity affect the frequency dependent of the measured optical polarization rotation angle: by creating a sharp feature near the plasma edge, which can be detected by experiments. Then we narrow down our research a bit further to the current induced magnetization.

In this thesis, I start with an introduction of some fundamental concepts and semi-classic transport theory which has been used through out this thesis. Then, I give a brief review of the recent development of Weyl semimetal, in which I show the purpose and concentration of our research. Chapter 3 and chapter 5 are the main parts of our research, which are published papers. Chapter 4 is, generally speaking, a glance of our current work. The appendices present Kubo formula derivations.

==> acknowledge.tex <==
 First, I would express my deepest and sincerest gratitude to my supervisor Prof. Dima Pesin, who guided me into this field of Weyl semimetal, helped me through every difficulty in my PhD life, infected me with a great passion for condensed matter research. During my doctoral study, I benefited a lot from his profound insight insight into physics. Second, I would like to thank my committee member Prof. Yongshi Wu, and Prof. Oleg Starykh. Prof. Wu  did a lot to persuade me that the condensed matter field would be a more promising field. He always tried to let me learn more about condensed matter theory, even when I was not that interested in it. Prof. Oleg is a fabulous teacher in the condensed matter theory. I owe most of my fundamental knowledge about condensed matter theory to the insistence of Prof. Wu, and the education received from Prof. Oleg. Finally, I would like to thank my colleagues Cuneyt \c{S}ahin and Janvida Rou. I learned a lot from many useful discussions with them. Last but not least, I need to thank the National Science Foundation for the financial support.
